Joint Manifold Learning and Density Estimation Using Normalizing Flows

Based on the manifold hypothesis, real-world data often lie on a low-dimensional manifold, while normalizing flows as a likelihood-based generative model are incapable of finding this manifold due to their structural constraints. So, one interesting question arises: $\textit{"Can we find sub-manifold(s) of data in normalizing flows and estimate the density of the data on the sub-manifold(s)?"}$. In this paper, we introduce two approaches, namely per-pixel penalized log-likelihood and hierarchical training, to answer the mentioned question. We propose a single-step method for joint manifold learning and density estimation by disentangling the transformed space obtained by normalizing flows to manifold and off-manifold parts. This is done by a per-pixel penalized likelihood function for learning a sub-manifold of the data. Normalizing flows assume the transformed data is Gaussianizationed, but this imposed assumption is not necessarily true, especially in high dimensions. To tackle this problem, a hierarchical training approach is employed to improve the density estimation on the sub-manifold. The results validate the superiority of the proposed methods in simultaneous manifold learning and density estimation using normalizing flows in terms of generated image quality and likelihood.

==> image_score.tex <==
\begin{tabular}{lccc}
		\toprule
		
		method & CIFAR10 & CelebA & LSUN (bedroom) \\
		\cmidrule{1-4}\morecmidrules\cmidrule{1-4}
		
		Baseline (Glow) & 3.35 & NA & 2.38\\
		Trained Glow & -& -\\
		\hline
		
		RealNVP & 3.49 & NA & 2.72 \\
		\hline
		
		DNF &  &  &  \\
		\hline
		
		Mflow &&& \\
		\hline
		
		Conformal & NA & NA & NA \\
		\hline

		Pixel Rejection & & 3.52 $\pm$ 0.04 & \\
		
% 		Pixel Rejection\#100 &  & \\
		
% 		Pixel Rejection (two step)\#100 && \\
% 		\hline
		
% 		PCA\#500 & - & 6.9e-04 $\pm$ 0.4e-03 & -\\
		
% 		PCA\#1000 & - &  1.6e-04 $ \pm $ 1.2e-04 & -\\
		
% 		PCA\#2000 & - & 1.e-05 $ \pm $ 1.e-05 & -\\
		
%		\hdashline
%		\hdashline

		
		\bottomrule
	\end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% #500 CelebA -> 0.01
% /hdd2/fatemeh/CelebA/FinalCode_GIT/MainFlow/ckpts_v28

% LEN(R) =>  857
% min =>  0.018533190712332726
% mean =>  0.022184182510492822
% median =>  0.022208932787179947
% max =>  0.02641185186803341
% std =>  0.001386739204823762

% LEN(BPD) =>  857
% min =>  3.389482238346474
% mean =>  3.5217240785000015
% median =>  3.522352365439862
% max =>  3.6802647716702825
% std =>  0.048101026478084015

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% #500 CelebA -> 0.001
% /hdd2/fatemeh/CelebA/FinalCode_GIT/MainFlow/ckpts_v29

% LEN(R) =>  857
% min =>  0.031283970922231674
% mean =>  0.0386099963423947
% median =>  0.03862546384334564
% max =>  0.0462927520275116
% std =>  0.0023215300047495385

% LEN(BPD) =>  857
% min =>  3.4112102971462805
% mean =>  3.543651453887192
% median =>  3.544526891201308
% max =>  3.7031203487291453
% std =>  0.04814447384158795

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% #500 CelebA -> 1.
% /hdd2/fatemeh/CelebA/FinalCode_GIT/MainFlow/ckpts_v26

% LEN(R) =>  857
% min =>  0.006896127015352249
% mean =>  0.007974694995372584
% median =>  0.007948052138090134
% max =>  0.009285259991884232
% std =>  0.00041436086981632916

% LEN(BPD) =>  857
% min =>  3.3912192631201887
% mean =>  3.524451034609363
% median =>  3.5249605396677466
% max =>  3.6834840575842334
% std =>  0.04800154207212458

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{tabular}{lccc}
% 		\toprule
		
% 		method & BPD & reconstruction error & FID \\
% 		\cmidrule{1-4}\morecmidrules\cmidrule{1-4}
		
% 		Baseline (Glow) & & - & -\\
% 		Trained Glow & & - & -\\
% 		\hline

% 		Proposed\#500 & & - &\\
		
% 		Proposed\#1000 & 3.80 $ \pm $ 0.01 & 0.01 $ \pm $ 0.3e-03 & todo: training\\
		
% 		Proposed\#2000 & 3.49 $\pm$ 0.01 & 0.005 $\pm$ 8.8e-05 & -\\
% 		\hline
		
% 		PCA\#500 & - & 6.9e-04 $\pm$ 0.4e-03 & -\\
		
% 		PCA\#1000 & - &  1.6e-04 $ \pm $ 1.2e-04 & -\\
		
% 		PCA\#2000 & - & 1.e-05 $ \pm $ 1.e-05 & -\\
		
% %		\hdashline
% %		\hdashline

		
% 		\bottomrule
% 	\end{tabular}

==> related_works.tex <==
\begin{tabular}{lcccccc}
		%\begin{tabular}{*5c}
		\toprule
		paper & loss & tract.density & optimization & manifold & chart & image \\ % \multicolumn{4}{c}{Car-Racing} & \multicolumn{4}{c}{Super-Mario}\\
		%\cmidrule(lr){2-4}\cmidrule(lr){5-7}
		%\midrule
		
		%\cline{1-5}
		%\cmidrule{1-6}		
		
		\cmidrule{1-7}\morecmidrules\cmidrule{1-7}
		
		%		\textbf{standard normalizing flow} & $L = \log p_{uv}(u,v) + \log \det J$ \\
		%		 & \\
		%		& \\
		%		\hline
		%		\textbf{flows for simultaneous manifold learning and density estimation} &  \\
		%		\textbf{SoftFlow: Probabilistic Framework for Normalizing Flow on Manifolds} &  \\
		%		\textbf{denoising normalizing flow} &  \\
		%		$L = \log$
		%		& \\
		%		\hline
		%		\textbf{Multi-chart flows} &  \\
		%		\textbf{Conformal Embedding Flows: Tractable Density Estimation on Learned Manifoldsw} &  \\
		%		\textbf{TRUMPETS: Injective Flows for Inference and Inverse Problemsw} &  \\
		
		GAN & 
		-
		& {\color{red} \xmark} & one-phase & learned & {\color{red} \xmark}  &  {\color{green} \cmark}  \\
		
		\hline
		VAE & 
		-
		& {\color{red} \xmark} & one-phase & learned & {\color{red} \xmark}  &  {\color{green} \cmark}  \\
		
		\hline
		NF & $\log p_{uv}(u,v) + \log\det J_f$ & {\color{green} \cmark} & one-phase & no &  {\color{red} \xmark}  &  {\color{green} \cmark} \\
		
		\hline
		M-flow & 
		\shortstack{
			$|| x-x'||=||x-f^{-1}(pad(select(f(x))))||$
			\\
			$\log P_{\hat{u}}(\hat{u}) + \log \det g + {\frac{1}{2}} \log \det (J_{f\circ pad}^TJ_{f\circ pad})$
		}
		& {\color{green} \cmark} & two-phase & learned &  {\color{green} \cmark}  &  {\color{red} \xmark}  \\
		
		\hline
		rectangular & 
		\shortstack{
			$ \log p_{\hat{u}} (\hat{u}) + \log \det J_g + \beta ||x - f^{-1}(pad(select(f(x))))||^2$
			\\
			$+ \frac{1}{2K} \sum_{k=1}^{K} stop-gradient (CG(J^T J; \epsilon_k)^T) J^T J \epsilon_k$
		}
		& {\color{green} \cmark} & one-phase & learned & {\color{green} \cmark}  &  ood  \\
		
		% todo: all cells
		\hline
		FOM & 
		-
		& - & - & prescribed & -  &  -  \\
		
		\hline
		PIE & 
		$\log p_{\hat{u}} + \log \det J_g + \log p_v(v) + \log \det J_f$
		& {\color{green} \cmark} & one-phase & learned & {\color{green} \cmark}  &  mnist  \\
		
		\hline
		multi-chart & 
		\shortstack{
			$|| x-x'||=||x-f^{-1}(pad(select(f(x))))||$
			\\
			$\log P_{\hat{u}}(\hat{u}) + \log \det g + {\frac{1}{2}} \log \det (J_{f_k\circ pad}^TJ_{f_k\circ pad})$
		}
		& {\color{green} \cmark} & two-phase & learned & {\color{green} \cmark}  &  {\color{red} \xmark}  \\
		
		\hline
		DNF &
		\shortstack{
			$\log p_{\hat{u}} + \log \det J_g + \log p_v(v) + \log \det J_f$
			\\
			$ + \lambda ||x-f^{-1}(pad(select(f(x))))||^2$
		}
		& {\color{green} \cmark} & one-phase & learned & {\color{green} \cmark}  &  celebA  \\
		
		\hline
		conformal & 
		$\log p_{\hat{u}}(\hat(u)) + \log \det J_g + d\lambda(u) + \alpha ||x - f(f^\dagger(x))||^2$
		& {\color{green} \cmark} & one-phase & learned & {\color{red} \xmark}  &  all  \\
		
		\hline
		trumpets & 
		\shortstack{
			$|| x-x'||=||x-f^\dagger(f(x))||$
			\\
			$\log P_{\hat{u}}(\hat{u}) + \log \det g$
		}
		& {\color{green} \cmark} & two-phase & learned & {\color{red} \xmark}  & {\color{red} \xmark}  \\
		
		\bottomrule
	\end{tabular}

%\begin{table}[h]
%%	\caption{Details of the most related researches.}
%%	\label{tab:loss}
%%	\setlength{\tabcolsep}{\tabcolsep}
%%	\centering
%%	%\color{red}
%%	%\begin{tabular}{c|c|cc|ccr}
%	\begin{tabular}{lcccccc}
%		%\begin{tabular}{*5c}
%		\toprule
%		paper & loss & tract.density & optimization & manifold & chart & image \\ % \multicolumn{4}{c}{Car-Racing} & \multicolumn{4}{c}{Super-Mario}\\
%		%\cmidrule(lr){2-4}\cmidrule(lr){5-7}
%		%\midrule
%		
%		%\cline{1-5}
%		%\cmidrule{1-6}		
%		
%		\cmidrule{1-7}\morecmidrules\cmidrule{1-7}
%		
%		%		\textbf{standard normalizing flow} & $L = \log p_{uv}(u,v) + \log \det J$ \\
%		%		 & \\
%		%		& \\
%		%		\hline
%		%		\textbf{flows for simultaneous manifold learning and density estimation} &  \\
%		%		\textbf{SoftFlow: Probabilistic Framework for Normalizing Flow on Manifolds} &  \\
%		%		\textbf{denoising normalizing flow} &  \\
%		%		$L = \log$
%		%		& \\
%		%		\hline
%		%		\textbf{Multi-chart flows} &  \\
%		%		\textbf{Conformal Embedding Flows: Tractable Density Estimation on Learned Manifoldsw} &  \\
%		%		\textbf{TRUMPETS: Injective Flows for Inference and Inverse Problemsw} &  \\
%		
%		GAN & 
%		-
%		& {\color{red} \xmark} & one-phase & learned & {\color{red} \xmark}  &  {\color{green} \cmark}  \\
%		
%		\hline
%		VAE & 
%		-
%		& {\color{red} \xmark} & one-phase & learned & {\color{red} \xmark}  &  {\color{green} \cmark}  \\
%		
%		\hline
%		NF & $\log p_{uv}(u,v) + \log\det J_f$ & {\color{green} \cmark} & one-phase & no &  {\color{red} \xmark}  &  {\color{green} \cmark} \\
%		
%		\hline
%		M-flow & 
%		\shortstack{
%			$|| x-x'||=||x-f^{-1}(pad(select(f(x))))||$
%			\\
%			$\log P_{\hat{u}}(\hat{u}) + \log \det g + {\frac{1}{2}} \log \det (J_{f\circ pad}^TJ_{f\circ pad})$
%		}
%		& {\color{green} \cmark} & two-phase & learned &  {\color{green} \cmark}  &  {\color{red} \xmark}  \\
%		
%		\hline
%		rectangular & 
%		\shortstack{
%			$ \log p_{\hat{u}} (\hat{u}) + \log \det J_g + \beta ||x - f^{-1}(pad(select(f(x))))||^2$
%			\\
%			$+ \frac{1}{2K} \sum_{k=1}^{K} stop-gradient (CG(J^T J; \epsilon_k)^T) J^T J \epsilon_k$
%		}
%		& {\color{green} \cmark} & one-phase & learned & {\color{green} \cmark}  &  ood  \\
%		
%		% todo: all cells
%		\hline
%		FOM & 
%		-
%		& - & - & prescribed & -  &  -  \\
%		
%		\hline
%		PIE & 
%		$\log p_{\hat{u}} + \log \det J_g + \log p_v(v) + \log \det J_f$
%		& {\color{green} \cmark} & one-phase & learned & {\color{green} \cmark}  &  mnist  \\
%		
%		\hline
%		multi-chart & 
%		\shortstack{
%			$|| x-x'||=||x-f^{-1}(pad(select(f(x))))||$
%			\\
%			$\log P_{\hat{u}}(\hat{u}) + \log \det g + {\frac{1}{2}} \log \det (J_{f_k\circ pad}^TJ_{f_k\circ pad})$
%		}
%		& {\color{green} \cmark} & two-phase & learned & {\color{green} \cmark}  &  {\color{red} \xmark}  \\
%		
%		\hline
%		DNF &
%		\shortstack{
%			$\log p_{\hat{u}} + \log \det J_g + \log p_v(v) + \log \det J_f$
%			\\
%			$ + \lambda ||x-f^{-1}(pad(select(f(x))))||^2$
%		}
%		& {\color{green} \cmark} & one-phase & learned & {\color{green} \cmark}  &  celebA  \\
%		
%		\hline
%		conformal & 
%		$\log p_{\hat{u}}(\hat(u)) + \log \det J_g + d\lambda(u) + \alpha ||x - f(f^\dagger(x))||^2$
%		& {\color{red} \xmark} & one-phase & learned & {\color{red} \xmark}  &  all  \\
%		
%		\hline
%		trumpets & 
%		\shortstack{
%			$|| x-x'||=||x-f^\dagger(f(x))||$
%			\\
%			$\log P_{\hat{u}}(\hat{u}) + \log \det g$
%		}
%		& {\color{green} \cmark} & two-phase & learned & {\color{red} \xmark}  & {\color{red} \xmark}  \\
%		
%		\bottomrule
%	\end{tabular}
%	%\end{table}
%\end{table}

==> scores.tex <==
\begin{tabular}{lccccccccc}
		\toprule
		
% 		\rotatebox{90}{method} & CIFAR10 & CelebA & LSUN (bedroom) \\
% 		\rotatebox{0}{criterion} 
% 		& \rotatebox{0}{DNF} 
% 		& \rotatebox{0}{Mflow} 
% 		& \rotatebox{0}{PR} 
% 		& \rotatebox{0}{E2E-H} 
% 		& \rotatebox{0}{E2E-M} 
% 		& \rotatebox{0}{H-HH}
% 		& \rotatebox{0}{H-HM}
% 		& \rotatebox{0}{H-MM}
% 		& \rotatebox{0}{H-MH}\\
		
		criterion
		& DNF
		& Mflow
		& PR
		& E2E-H
		& E2E-M
		& H-HH
		& H-HM
		& H-MM
		& H-MH\\
		
		\cmidrule{1-10}\morecmidrules\cmidrule{1-10}
		FID & 58.61 &1& 78.65 & 71.61 & 59.84 & 101.57 & 101.22 &102.09&98.73 \\
		RE & 0.004 $\pm$ 0.0002  &1& 0.02 $\pm$ 0.001 &  0.02 $\pm$ 0.001  &  0.005 $\pm$ 0.0002 &0.05 $\pm$ 0.004 & 0.05 $\pm$ 0.004 & 0.05 $\pm$ 0.004 & 0.05 $\pm$ 0.004 \\
		BPD & 3.98 $\pm$ 0.03  &1& 3.52 $\pm$ 0.04 & 3.53 $\pm$ 0.05 & 3.51 $\pm$ 0.05 &  3.51 $\pm$ 0.05   & 3.51 $\pm$ 0.05 & 3.47 $\pm$ 0.05 & 3.48 $\pm$ 0.05 \\
% 		\hline
% 		FID
% 		RE
% 		BPD
		
		
% %		\hdashline
% %		\hdashline

		
		\bottomrule
	\end{tabular}

%% PATH
% /hdd2/fatemeh/CelebA/FinalCode_GIT/pure_DNF
